Super $q$-Howe duality and web categories

We use super $q$-Howe duality to provide diagrammatic presentations of an idempotented form of the Hecke algebra and of categories of $\mathfrak{gl}_N$-modules (and, more generally, $\mathfrak{gl}_{N|M}$-modules) whose objects are tensor generated by exterior and symmetric powers of the vector representations. As an application, we give a representation theoretic explanation and a diagrammatic version of a known symmetry of colored HOMFLY--PT polynomials.

==> defs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              %
% Commands, definitions        %
% and styles                   %
%                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{latexsym,exscale,enumerate,enumitem,amsfonts,mathtools}
\usepackage{amsfonts,amscd,stmaryrd,textcomp,xcolor}
\usepackage{amssymb}
\usepackage[normalem]{ulem}
\usepackage{young,youngtab}
\usepackage{thmtools}
\usepackage{easybmat}
\usepackage{pinlabel}
%\usepackage{draftwatermark}%Remove it later!
%\SetWatermarkScale{6}%Remove it later!

%\usepackage{datetime}%Remove it later!

\addtolength{\hoffset}{-1.6cm}
\addtolength{\textwidth}{3cm}

\usepackage[all]{xy}
\SelectTips{cm}{}


\usepackage{tikz}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows,shapes,positioning}
%%multiple arrow options
\tikzstyle directed=[postaction={decorate,decoration={markings,
    mark=at position #1 with {\arrow{>}}}}]
\tikzstyle rdirected=[postaction={decorate,decoration={markings,
    mark=at position #1 with {\arrow{<}}}}]
\tikzset{anchorbase/.style={baseline={([yshift=-0.5ex]current bounding box.center)}},
}
    
\newcommand{\qbin}[2]{{\textstyle\genfrac{[}{]}{0pt}{}{#1}{#2}}}
\newcommand{\qbinn}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}
    
\newcommand{\comm}[1]{}
\def\cal#1{\mathcal{#1}}%
\newcommand{\sln}{\mathfrak{sl}_N}
\newcommand{\slnn}[1]{\mathfrak{sl}_{#1}}
\newcommand{\gln}{\mathfrak{gl}_N}
\newcommand{\glm}{\mathfrak{gl}_m}
\newcommand{\glmn}{\mathfrak{gl}_{m|n}}
\newcommand{\glMN}{\mathfrak{gl}_{N|M}}
\newcommand{\glNM}{\mathfrak{gl}_{M|N}}
\newcommand{\glnn}[1]{\mathfrak{gl}_{#1}}
\newcommand{\bV}{\raisebox{0.03cm}{\mbox{\footnotesize$\textstyle{\bigwedge}$}}}
\newcommand{\bW}{\bigwedge}
\newcommand{\Gam}{\Gamma_{N}}
\newcommand{\Gami}{\Gamma_{\In}}
\newcommand{\Gams}{\Gamma_{N}^{\mathrm{sort}}}
\newcommand{\Lad}{\Upsilon^{m|n}_{\mathrm{su}}}
\newcommand{\AltSp}{N\text{-}\!\textbf{Web}_{\mathrm{g}}}
\newcommand{\CKM}{N\text{-}\!\textbf{Web}_{\mathrm{CKM}}}
\newcommand{\SymSp}{N\text{-}\!\textbf{Web}_{\mathrm{r}}}
\newcommand{\Sp}[2]{{#1}\text{-}\!\textbf{Web}_{\mathrm{{#2}}}}
\newcommand{\SuSp}{N\text{-}\!\textbf{Web}_{\mathrm{gr}}}
\newcommand{\MNSp}{N|M\text{-}\!\textbf{Web}_{\mathrm{gr}}}
\newcommand{\InSp}{\In\text{-}\!\textbf{Web}_{\mathrm{gr}}}
\newcommand{\InSpf}{\In\text{-}\!\textbf{Web}_{\mathrm{gr}}^f}
\newcommand{\SoSuSp}{N\text{-}\!\textbf{Web}_{\mathrm{gr}}^{\mathrm{sort}}}
\newcommand{\SoInSp}{\In\text{-}\!\textbf{Web}_{\mathrm{gr}}^{\mathrm{sort}}}
\newcommand{\SoMNSp}{N|M\text{-}\!\textbf{Web}_{\mathrm{gr}}^{\mathrm{sort}}}
\newcommand{\Alt}{\mathrm{Ext}}
\newcommand{\Sym}{\mathrm{Sym}}
\newcommand{\Sup}{\bullet}
\newcommand{\Su}{\mathrm{su}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\triv}{\;\raisebox{-0.02cm}{\mbox{{\tiny$\yng(2)$}}\;}}
\newcommand{\sign}{\;\raisebox{0.05cm}{\mbox{{\tiny\Yvcentermath1$\yng(1,1)$}}\;}}
\newcommand{\onesign}{\;\raisebox{0.05cm}{\mbox{{\tiny\Yvcentermath1$\yng(1)$}}\;}}
\newcommand{\exti}{\;\raisebox{.35cm}{\raisebox{-0.02cm}{\mbox{{\tiny$\yng(1)$}}\;}
\hspace*{-.425cm}\raisebox{-0.4cm}{\vdots}
\hspace*{-.45cm}
\raisebox{-0.75cm}{\mbox{{\tiny$\yng(1)$}}\;}}
}
\newcommand{\symi}{\;\raisebox{0.05cm}{\mbox{{\tiny\Yvcentermath1$\yng(1)$}}}\cdots
\raisebox{0.05cm}{\mbox{{\tiny\Yvcentermath1$\yng(1)$}}\;}}

\newcommand{\Uu}{\textbf{U}}
\newcommand{\Uq}{\textbf{U}_q}
\newcommand{\Ud}{\dot{\textbf{U}}_q}
\newcommand{\Us}{\textbf{U}_q(\glmn)}
\newcommand{\Usu}{\textbf{U}_q(\glMN)}
\newcommand{\Usd}{\dot{\textbf{U}}_q(\glmn)}
\newcommand{\Uun}{\textbf{U}_q(\mathfrak{gl}_N)}
\newcommand{\Ut}{\tilde{\textbf{U}}_q(\mathfrak{gl}_N)}
\newcommand{\He}{\textbf{H}}
\newcommand{\Hee}{\check{\textbf{H}}}
\newcommand{\Repn}{\mathfrak{gl}_{N}\text{-}\textbf{fdMod}}
\newcommand{\Repe}[1]{\mathfrak{gl}_{{#1}}\text{-}\textbf{Mod}_{e}}
\newcommand{\Reps}[1]{\mathfrak{gl}_{{#1}}\text{-}\textbf{Mod}_{s}}
\newcommand{\Repas}{\mathfrak{gl}_{N}\text{-}\textbf{Mod}_{\mathrm{es}}}
\newcommand{\Repsas}{\mathfrak{gl}_{N}\text{-}\textbf{Mod}^{\mathrm{sort}}_{\mathrm{es}}}
\newcommand{\RepMN}{\mathfrak{gl}_{N|M}\text{-}\textbf{Mod}_{\mathrm{es}}}
\newcommand{\RepMNs}{\mathfrak{gl}_{N|M}\text{-}\textbf{Mod}^{\mathrm{sort}}_{\mathrm{es}}}
\newcommand{\repn}{\mathfrak{sl}_{N}\text{-}\textbf{fdMod}}
\newcommand{\repe}[1]{\mathfrak{sl}_{{#1}}\text{-}\textbf{Mod}_{e}}
\newcommand{\reps}[1]{\mathfrak{sl}_{{#1}}\text{-}\textbf{Mod}_{s}}
\newcommand{\repas}{\mathfrak{sl}_{N}\text{-}\textbf{Mod}_{\mathrm{es}}}
\newcommand{\repsas}{\mathfrak{sl}_{N}\text{-}\textbf{Mod}^{\mathrm{sort}}_{\mathrm{es}}}
\newcommand{\Kar}{\textbf{Kar}}
\newcommand{\Mat}{\textbf{Mat}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\End}{\mathrm{End}}
\newcommand{\nn}{N}
\newcommand{\In}{\infty}
\newcommand{\grre}{{}_{\mathrm{gr}}}
\newcommand{\gr}{{}_{\mathrm{g}}}
\newcommand{\re}{{}_{\mathrm{r}}}


\newcommand{\Inw}{\In\text{-}\!\textbf{Web}^{\mathrm{sort}}_{m+n}}
\newcommand{\MNw}{N|M\text{-}\!\textbf{Web}^{\mathrm{sort}}_{m+n}}
\newcommand{\MNr}{\mathfrak{gl}(N|M)\text{-}\textbf{Mod}^{\mathrm{sort}}_{m+n}}


\newcommand{\brac}[2]{\left\langle {#1}\right\rangle_{{#2}}}

\def\C{{\mathbb C}}
\def\Cq{{\mathbb C}_{\tilde q}}
\def\Ca{{\mathbb C}_{a,q}}
\def\N{{\mathbb N}}
\def\Z{{\mathbb Z}}
\def\Zg{{\mathbb{Z}_{\geq 0}}}
\def\Q{{\mathbb Q}}
\def\K{{\mathbb K}}
\def\R{{\mathbb R}}


\def\one{\mathrm{1}}


% THEOREMS -------------------------------------------------------
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}

\theoremstyle{definition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{nota}[thm]{Notation}
\newtheorem{as}[thm]{Assumption}
%\newtheorem{ex}[thm]{Example}
%\newtheorem{exa}[thm]{Example/Convention}
\newtheorem*{thmm}{Theorem}
\newtheorem*{propp}{Proposition}

\declaretheorem[style=definition,name=Example,qed=$\blacksquare$,numberlike=thm]{ex}
\declaretheorem[style=definition,name=Definition,qed=$\Diamond$,numberlike=thm]{defn}

\numberwithin{equation}{section}

\definecolor{mycolor}{rgb}{0.9,0,0}
\definecolor{orchid}{RGB}{143,40,194}
\definecolor{lava}{RGB}{207,16,32}

%qed=$\blacksquare$

% maintenance
\def\DT#1{\textcolor[rgb]{0.00,1.00,0.00}{#1}}%
\def\PV#1{\textcolor[rgb]{0.00,0.00,1.00}{#1}}%
\def\PW#1{\textcolor[rgb]{1.00,0.00,0.00}{#1}}%

\setcounter{tocdepth}{2}
\setcounter{secnumdepth}{3}
\numberwithin{equation}{section}
\usepackage[final]{hyperref, bookmark}
\usepackage{cleveref}
\hypersetup{
    pdftoolbar=true,        
    pdfmenubar=true,        
    pdffitwindow=false,     
    pdfstartview={FitH},    
    pdftitle={Super \texorpdfstring{$q$}{q}-Howe duality and web categories},    
    pdfauthor={Daniel Tubbenhauer, Pedro Vaz and Paul Wedrich},     
    pdfsubject={},   
    pdfcreator={Daniel Tubbenhauer, Pedro Vaz and Paul Wedrich},   
    pdfproducer={Daniel Tubbenhauer, Pedro Vaz and Paul Wedrich}, 
    pdfkeywords={}, 
    pdfnewwindow=true,      
    colorlinks=true,       
    linkcolor=lava,          
    citecolor=teal,        
    filecolor=magenta,      
    urlcolor=orchid,          
    linkbordercolor=lava,
    citebordercolor=teal,
    urlbordercolor=orchid,  
    linktocpage=true
}

%
\let\fullref\autoref
%  To work correctly the environment name must have a corrresponding 
%  \XXXautorefname defined.  The following command does the job:
%
\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}
%
%  Some standard autorefnames.  If the environment name for an autoref 
%  you need is not listed below, add a similar line to your TeX file:
%  
\makeautorefname{equation}{Equation}%
\makeautorefname{footnote}{footnote}%
\makeautorefname{item}{item}%
\makeautorefname{figure}{Figure}%
\makeautorefname{table}{Table}%
\makeautorefname{part}{Part}%
\makeautorefname{appendix}{Appendix}%
\makeautorefname{chapter}{Chapter}%
\makeautorefname{section}{Section}%
\makeautorefname{subsection}{Section}%
\makeautorefname{subsubsection}{Section}%
\makeautorefname{paragraph}{Paragraph}%
\makeautorefname{subparagraph}{Paragraph}%
\makeautorefname{theorem}{Theorem}%
\makeautorefname{theo}{Theorem}%
\makeautorefname{thm}{Theorem}%
\makeautorefname{addendum}{Addendum}%
\makeautorefname{addend}{Addendum}%
\makeautorefname{add}{Addendum}%
\makeautorefname{maintheorem}{Main theorem}%
\makeautorefname{mainthm}{Main theorem}%
\makeautorefname{corollary}{Corollary}%
\makeautorefname{corol}{Corollary}%
\makeautorefname{coro}{Corollary}%
\makeautorefname{cor}{Corollary}%
\makeautorefname{lemma}{Lemma}%
\makeautorefname{lemm}{Lemma}%
\makeautorefname{lem}{Lemma}%
\makeautorefname{sublemma}{Sublemma}%
\makeautorefname{sublem}{Sublemma}%
\makeautorefname{subl}{Sublemma}%
\makeautorefname{proposition}{Proposition}%
\makeautorefname{proposit}{Proposition}%
\makeautorefname{propos}{Proposition}%
\makeautorefname{propo}{Proposition}%
\makeautorefname{prop}{Proposition}%
\makeautorefname{property}{Property}
\makeautorefname{proper}{Property}
\makeautorefname{scholium}{Scholium}%
\makeautorefname{step}{Step}%
\makeautorefname{conjecture}{Conjecture}%
\makeautorefname{conject}{Conjecture}%
\makeautorefname{conj}{Conjecture}%
\makeautorefname{question}{Question}
\makeautorefname{questn}{Question}
\makeautorefname{quest}{Question}
\makeautorefname{ques}{Question}
\makeautorefname{qn}{Question}
\makeautorefname{definition}{Definition}%
\makeautorefname{defin}{Definition}%
\makeautorefname{defi}{Definition}%
\makeautorefname{def}{Definition}%
\makeautorefname{dfn}{Definition}%
\makeautorefname{notation}{Notation}
\makeautorefname{nota}{Notation}
\makeautorefname{notn}{Notation}
\makeautorefname{remark}{Remark}%
\makeautorefname{rema}{Remark}%
\makeautorefname{rem}{Remark}%
\makeautorefname{rmk}{Remark}%
\makeautorefname{rk}{Remark}%
\makeautorefname{remarks}{Remarks}%
\makeautorefname{rems}{Remarks}%
\makeautorefname{rmks}{Remarks}%
\makeautorefname{rks}{Remarks}%
\makeautorefname{example}{Example}%
\makeautorefname{examp}{Example}%
\makeautorefname{exmp}{Example}%
\makeautorefname{exam}{Example}%
\makeautorefname{exa}{Example}%
\makeautorefname{algorithm}{Algorith}%
\makeautorefname{algo}{Algorith}%
\makeautorefname{alg}{Algorith}%
\makeautorefname{axiom}{Axiom}%
\makeautorefname{axi}{Axiom}%
\makeautorefname{ax}{Axiom}%
\makeautorefname{case}{Case}%
\makeautorefname{claim}{Claim}%
\makeautorefname{clm}{Claim}%
\makeautorefname{assumption}{Assumption}%
\makeautorefname{assumpt}{Assumption}%
\makeautorefname{conclusion}{Conclusion}%
\makeautorefname{concl}{Conclusion}%
\makeautorefname{conc}{Conclusion}%
\makeautorefname{condition}{Condition}%
\makeautorefname{condit}{Condition}%
\makeautorefname{cond}{Condition}%
\makeautorefname{construction}{Construction}%
\makeautorefname{construct}{Construction}%
\makeautorefname{const}{Construction}%
\makeautorefname{cons}{Construction}%
\makeautorefname{criterion}{Criterion}%
\makeautorefname{criter}{Criterion}%
\makeautorefname{crit}{Criterion}%
\makeautorefname{exercise}{Exercise}%
\makeautorefname{exer}{Exercise}%
\makeautorefname{exe}{Exercise}%
\makeautorefname{problem}{Problem}%
\makeautorefname{problm}{Problem}%
\makeautorefname{probm}{Problem}%
\makeautorefname{prob}{Problem}%
\makeautorefname{solution}{Solution}%
\makeautorefname{soln}{Solution}%
\makeautorefname{sol}{Solution}%
\makeautorefname{summary}{Summary}%
\makeautorefname{summ}{Summary}%
\makeautorefname{sum}{Summary}%
\makeautorefname{operation}{Operation}%
\makeautorefname{oper}{Operation}%
\makeautorefname{observation}{Observation}%
\makeautorefname{observn}{Observation}%
\makeautorefname{obser}{Observation}%
\makeautorefname{obs}{Observation}%
\makeautorefname{ob}{Observation}%
\makeautorefname{convention}{Convention}%
\makeautorefname{convent}{Convention}%
\makeautorefname{conv}{Convention}%
\makeautorefname{cvn}{Convention}%
\makeautorefname{warning}{Warning}%
\makeautorefname{warn}{Warning}%
\makeautorefname{note}{Note}%
\makeautorefname{fact}{Fact}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{showkeys}%%%%%                                                                         i've enabled showkeys...we'll turn it off before the arxiv!                                 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

